Superconductivity in heavy fermion compounds

We review the current state of experimental and theoretical investigations of heavy fermion superconductors. We discuss most of the Ce-based compounds like Ce122, Ce115, Ce218 and Ce131 classes and U-based superconductors like UBe_13 and UPd_2Al_3. In the former the emphasis is on the connection to quantum critical phenomena and non-Fermi liquid behaviour. Recent neutron scattering and hydrostatic pressure results on SDW/SC competition in the Ce122 system are included. For the U-compounds we discuss the significance of dual models with both localised and itinerant 5f electrons for mass enhancement and superconducting pair formation. Itinerant spin fluctuation theories for unconventional superconductivity are also reviewed.

==> 0acronym.tex <==
%auto-ignore
\begin{table}[hbtp]
{\em List of acronyms}\\[0.5cm]

\begin{tabular}{ll}
AF     &   antiferromagnet, antiferromagnetism, antiferromagnetic\\
ARPES  &   angle resolved photoemission spectroscopy\\
BIS    &   bremsstrahlung isochromat spectroscopy\\
BZ     &   Brillouin zone\\
CDW    &   charge density wave\\
CEF    &   crystalline electric field\\
dHvA   &   de Haas-van Alphen\\
DLRO   &   diagonal long range order\\
DOS    &   density of states\\
FFLO   &   Fulde-Ferrell-Larkin-Ovchinnikov\\
LFL    &   Landau-Fermi liquid\\
FLEX   &   fluctuation exchange\\
FM     &   ferromagnet, ferromagnetism, ferromagnetic\\
FS     &   Fermi surface\\
HF     &   heavy fermion\\
IC     &   incommensurate\\
INS    &   inelastic neutron scattering\\
LDA    &   local density approximation\\
LSDA   &   local spin density approximation\\
mf     &   mean field\\
NFL    &   non-Fermi liquid\\
n.n.   &   next neighbor\\ 
n.n.n. &   next nearest neighbor\\
NCA    &   non-crossing approximation\\
NMR    &   nuclear magnetic resonance\\
ODLRO  &   off-diagonal long range order\\
OP     &   order parameter\\
PES    &   photoemission spectroscopy\\
QCP    &   quantum critical point\\
qp     &   quasi particle\\
RPA    &   random phase approximation\\
RKKY   &   Ruderman-Kittel-Kasuya-Yoshida\\
SC     &   superconductor, superconductivity, superconducting\\
SDW    &   spin density wave\\
s.o.   &   spin orbit\\
\end{tabular}
\end{table}

==> header.tex <==
%auto-ignore
\begin{center}
To be published in\\[0.3cm]
\bf
A. Narlikar (Ed.)\\
``Frontiers in Superconducting Materials''\\
Springer Verlag, Berlin, 2004
\rm
\end{center}
